Distributed Active State Estimation with User-Specified Accuracy

In this paper, we address the problem of controlling a network of mobile sensors so that a set of hidden states are estimated up to a user-specified accuracy. The sensors take measurements and fuse them online using an Information Consensus Filter (ICF). At the same time, the local estimates guide the sensors to their next best configuration. This leads to an LMI-constrained optimization problem that we solve by means of a new distributed random approximate projections method. The new method is robust to the state disagreement errors that exist among the robots as the ICF fuses the collected measurements. Assuming that the noise corrupting the measurements is zero-mean and Gaussian and that the robots are self localized in the environment, the integrated system converges to the next best positions from where new observations will be taken. This process is repeated with the robots taking a sequence of observations until the hidden states are estimated up to the desired user-specified accuracy. We present simulations of sparse landmark localization, where the robotic team achieves the desired estimation tolerances while exhibiting interesting emergent behavior.

==> reviews-response/comm-complexity.tex <==
The communication complexity of the consensus part is essentially the same as any consensus algorithm.
Each robot has to send $\bbz$, $\bbxi$, and $\bbXi$ to its neighbors.
The sizes of each of these objects are $pn,$ $qm,$ and $\frac{qm(qm+1)}{2}.$
The total number of messages, i.e., the max value of $k$ can be specified ahead of time and is limited by the length of the time interval between $t-1$ and $t$.

We have analytical expressions for the gradient, so its not clear how to include formally a measure of computational complexity.
The robot simply evaluates a closed form function to find a search direction.
The most complex operations are the eigendecomposition of a $p \times p$ symmetric matrix, done in $O(p^3)$ time.

==> reviews-response/johansson08-discuss.tex <==
%Relevant also is the subgradient projection algorithm in \cite{johansson08} because it appears to be the only other work that formally takes into account disagreement errors due to incomplete consensus.
%Our algorithm and analysis is focussed on problems with many constraints, where the simple projection in \cite{johansson08} may be slow, so it requires a different set of tools for analysis and therefore the suboptimality bounds in \cite{johansson08} may not directly apply.
%
%While \cite{johansson08} bounds on the sub optimality due to interleaving consensus and optimization, 
%
%While there are known suboptimality bounds for such algorithms \cite{johansson08}, 

==> reviews-response/nonlocal.tex <==
Although the objective function \eqref{eq:sep_obj} is separable and the constraints \eqref{eq:LMI2} are linear in $\bbz_s$, the problem is not readily distributed because the presence of $\ccalD$ couples all sensors in the network; cf. \eqref{eq:if-map}.
In what follows, we present an algorithm that assigns each agent a local copy of the data $\ccalD_s$ that may disagree with other nodes.
The algorithm interleaves the ICF with optimization, so that each $\ccalD_s$ progresses towards a common consensus value.
Recalling that this process is occurring during the interval $[t-1, t],$ the consensus value for the data is $\ccalD(t)$.

==> reviews-response/objective-correction.tex <==
We apologize for this error.
The comments are completely valid. 
We've removed the boldface for $\gamma_i$ since it is scalar.
We've also removed the ${\rm min}$ function from the objective, as it is unnecessary, as the reviewer points out here and as R12 points out in Point Raised~\ref{minimax12}.

==> reviews-response/pde.tex <==
We note also that active sensors also have great potential for solving the most difficult problems in estimation, inverse problems for PDE-constrained systems \cite{patan12, khodayi15}.
Our focus is on low-cost network coordination, which, to our knowledge, is only currently possible at the scales, measured both in terms of the number of sensors and hidden states, considered in this paper under our simpler model.

==> reviews-response/previous.tex <==
Compared to the work in \cite{lee15distributed,Soomin-report2}, we made the following nontrivial modifications. 
\begin{enumerate}[(a)]
\item Since the consensus and optimization have to be done in parallel, the constraint functions $h$ depend on time, and therefore, the problem itself evolves as the algorithm proceeds. To handle this evolving disagreement error in the constraint functions, we had to find a new iterate relation (Lemma V.7) with the error terms $\delta_{s,k}$ and $\nu_{s,k}$.
\item All the proofs in Appendix A are devoted to show that these error sequences $\{\delta_{s,k}\}$ and $\{\nu_{s,k}\}$ are summable.
\item Even with the summability, these additional terms lead us to group all the terms in Lemma V.7 more carefully for showing the asymptotic feasibility and network disagreement. 
\end{enumerate}

==> reviews-response/sensor-selection.tex <==
%One key difference between our work and \cite{JoshiBoyd09, ranieri14, chepuri14} is that we control motion whereas those works select sensors from a discrete set.
%Each problem has unique challenges, which is why we focussed on literature review on approaches that control in continuous domains \cite{chung06,jalalkamali12,freundlich13cdc,freundlich15acc, freundlich13icra,vanderhook15}.
%Some works do bridge the gap, e.g., \cite{JoshiBoyd09} addresses sensor scheduling by making a convex relaxation of the integer constraints, however this aproach generally does not perform as well as integer programming appraoches, such as \cite{ranieri14, chepuri14}.
%Worst case estimation has also been addressed from a signal processing persepctive \cite{JoshiBoyd09, ranieri14, chepuri14, jamali15,simonetto16}, where the goal is to select sensors or observations from a discrete set.
We note here that \cite{JoshiBoyd09} suggests a convex relaxation of the integer constraints for sensor scheduling, however this aproach is not guarunteed to outperform integer programming \cite{ ranieri14, chepuri14} for the selection problem.

==> reviews-response/stationary.tex <==
%In our initial manuscript, we thought it was obvious that the proofs would go through with the terms $A, C$ and $\bbchi$.
%While we think it is likely that our proofs will hold, we agree that it is not obvious based on the derivations in the paper and appendices.
%We leave the potentially nontrivial task of proving it to future work.
%In the revision, we limit our claims to the model in \eqref{1ap} and \eqref{1bp}.
%
%We have also removed Remark II.1 from the original submission, since it no longer makes sense without the original linear system.
In the revision, we have defined only terms that are critical to the proofs and the approach.
Therefore, we do not define $A, C$, or $\chi$ in the revision.
We thank the reviewer for this comment, as it has enabled us to eliminate several unnecessary variables.
%, vastly simplifying our exposition, ultimately leading to an improved exposition of our ideas.
%We also add that it is likely that our derivations would hold for a more general linear system such as the one defined in the first submission, but we leave the potentially nontrivial task of proving it to future work.

We have also removed Remark II.1 from the original submission, since it no longer makes sense without the original linear system.

==> reviews-response/whole-scene.tex <==
Yes, each sensor gets the ``whole picture'' of the environment at every observation time.
However, we only require the information model to have bounded first and second derivatives, so an information model that is identically $\bb0$ after some finite range or viewing angle is allowed.
A measurement with $\bb0$ information will be correctly ignored by the filter.
We have added a brief explanation to this effect in the first column of Section 2.

==> text-16p/unused/derivs.tex <==
%For notational purposes, let $\iota (s,j)$ be an indicator function such that 
%\begin{equation}
%\iota_s^j
%=
%\begin{cases}
%1&{{\rm if}} \; 2s = j
%\\
%2&{{\rm if}} \; 2s + 1 = j
%\\
%0&{{\rm else}} 
%\end{cases}
%\end{equation}
\begin{prop}
The derivatives of the information matrix with respect to the control input $\frac{\partial Q_{i,s}}{\partial [u_v]_j}$ is the zero matrix if $s \neq v$, and if $s=v$, then
\begin{align*}
 \frac{\partial Q_{i,s}}{\partial [u_s]_j}  
&=
\begin{cases}
\begin{matrix}
([\hhatx_{i,s}]_2 - [r_s]_2-[u_s]_2)
X_{i,s}
\\
\qquad+
([\hhatx_{i,s}]_1 - [r_s]_1-[u_s]_1) Y_{i,s}
\end{matrix}
 &{{\rm if}} \; j=1
\\
\begin{matrix}
([r_s]_1+[u_s]_1 - [\hhatx_{i,s}]_1)X_{i,s}
\\
\qquad+
([\hhatx_{i,s}]_2 - [r_s]_2 - [u_s]_2) Y_{i,s}
\end{matrix}
&{{\rm if}} \;   j=2
\end{cases}
\end{align*}
where
\agn*{
X_{i,s} &= 
\frac{(1-\rho) \lambda_{1,i,s}}{\norm{\hhatx_{i,s}-r_s-u_s}^2}
 \mat{ 
- \sin 2\phi_{i,s} &
 \cos 2 \phi_{i,s} \\ 
  \cos 2 \phi_{i,s}  &
   \sin 2 \phi_{i,s} 
} \and
\\
Y_{i,s} &= 
\left(  \frac{  c_0c_1 }{ \left(1 + c_1\norm{\hhatx_{i,s}-r_s-u_s}\right)^{2} \norm{\hhatx_{i,s}-r_s-u_s}} \right) \\
&\hspace{1cm} *
\mat{  
(1-\rho)\cos^2 \phi_{i,s}  + \rho  &
\frac{1}{2} (1-\rho)\sin 2 \phi_{i,s}  \\ 
\frac{1}{2} (1-\rho)\sin 2 \phi_{i,s}  &
(\rho-1)\cos^2 \phi_{i,s}  +1 
}.
}
Note that $\lambda_{1,i,s}$ and $\phi_{i,s}$ are functions os $\hhatx_{i,s}$ and $r_s + u_s$, given in equations \eqref{eq:phi} and \eqref{eq:lambdas}.
\end{prop}

%\begin{prop}
%The derivatives of the entries of the Laplacian matrix $L(r+u) = (\ell_{sv})$ with respect to the control inputs $j = 1, \dots, 2n$ by
%\agn*{
%\frac{\partial \ell_{sv} }{\partial u_j} = 
%\begin{cases}
%\sum_{k \in \ccalV} \frac{\partial a_{sk}}{\partial u_j}  &{{\rm if}} \; s=v\\
%-\frac{\partial a_{sv}}{\partial u_j}  &{{\rm else}} \; 
%\end{cases}
%}
%where 
%\agn*{
%\frac{\partial a_{sv}}{\partial u_j} &=  - \frac{\partial \sigma_w }{\partial y} \big|_{y = \epsilon - d_{sv} (r + u)} \frac{\partial d_{sv}}{\partial u_j},
%\\
%\frac{\partial \sigma_w }{\partial y}  
%&=
%\frac{ -we^{-wy}}{(1 - e^{-wy})^{2} },
%\and
%\\
% \frac{\partial d_{sv}}{\partial u_j}
% &=\begin{cases}
%\frac{1}{ d_{sv}}([r_s]_1 + [u_s]_1 - [r_v]_1 - [u_v]_1 )&{{\rm if}} \iota_s^j = 1 \; 
% \\
%\frac{1}{ d_{sv}}([r_s]_2 + [u_s]_2 - [r_v]_2 - [u_v]_2 ) &{{\rm if}} \iota_s^j = 2 \; 
%\\
%\frac{1}{ d_{sv}}([r_v]_1 + [u_v]_1 - [r_s]_1 - [u_s]_1 )&{{\rm if}} \iota_v^j = 1 \; 
% \\
%\frac{1}{ d_{sv}}([r_v]_2 + [u_v]_2 - [r_s]_2 - [u_s]_2 )&{{\rm if}} \iota_v^j = 2 \; 
%\\
%0 &{{\rm else}}
% \end{cases}
%}
%\end{prop}
%\begin{proof}
%Recall that $L(r + u) = \Delta(r + u) - A(r + u)$ where $\Delta \triangleq \diag ( \sum_{v \in \ccalV} a_{sv}).$
%Consider one component of $L$, given by by $(\ell_{sv})$, and one component of the control input $u_j$.
%We have that
%\agn*{
%\frac{\partial \ell_{sv} }{\partial u_j} = 
%\begin{cases}
%\sum_{k \in \ccalV} \frac{\partial a_{sk}}{\partial u_j}  &{{\rm if}} \; s=v\\
%-\frac{\partial a_{sv}}{\partial u_j}  &{{\rm else}} \; 
%\end{cases}
%}
%From the chain rule and the definition of the adjacency matrix in \eqref{eq:sigmoid}, we have that
%\[
%\frac{\partial a_{sv}}{\partial u_j} =  - \frac{\partial \sigma_w }{\partial y} \big|_{y = \epsilon - d_{sv} (r + u)} \frac{\partial d_{sv}}{\partial u_j},
%\]
%and we recall that $\epsilon$ and $w$ are user-specified constants.
%From elementary calculus, 
%\[
%\frac{\partial \sigma_w }{\partial y}  =
%\frac{\partial  }{\partial y}(1 - e^{-wy})^{-1}
%=
%\frac{ -we^{-wy}}{(1 - e^{-wy})^{2} }.
%\]
%The remaining derivatives are given by
%\begin{align*}
% \frac{\partial d_{sv}}{\partial u_j}
% =\begin{cases}
%\frac{1}{ d_{sv}}([r_s]_1 + [u_s]_1 - [r_v]_1 - [u_v]_1 )&{{\rm if}} \iota_s^j = 1 \; 
% \\
%\frac{1}{ d_{sv}}([r_s]_2 + [u_s]_2 - [r_v]_2 - [u_v]_2 ) &{{\rm if}} \iota_s^j = 2 \; 
%\\
%\frac{1}{ d_{sv}}([r_v]_1 + [u_v]_1 - [r_s]_1 - [u_s]_1 )&{{\rm if}} \iota_v^j = 1 \; 
% \\
%\frac{1}{ d_{sv}}([r_v]_2 + [u_v]_2 - [r_s]_2 - [u_s]_2 )&{{\rm if}} \iota_v^j = 2 \; 
%\\
%0 &{{\rm else}}
% \end{cases}
%\end{align*}
%\end{proof}

%The second derivatives of the Lagrangian with respect to the primal variables is given component wise by
%\begin{align}\label{eq:primalHessian}
%\frac{\partial^2 \ccalL }{\partial u_j \partial u_k}
%&=
%-\sum_{i=1}^{m}  \Omega_i   \left( \sum_{s \in \ccalN_s}  \frac{\partial^2 Q_{i,s}}{\partial u_j \partial u_k}   \right)
%\\
%&\hspace{1cm}
%-
%\Omega_{m+1}  (I - \frac{2}{n}{\bf 1}{\bf 1}^\top)  \frac{\partial^2 L}{\partial u_j \partial u_k} \nonumber
%\\
%\and \frac{\partial^2 \ccalL }{\partial \gamma_j \partial \gamma_k} &= 0.\nonumber
%\end{align}
%The second derivatives that appear in \eqref{eq:primalHessian} are given in the following two propositions.
%The proofs are given in the appendix.

\begin{prop}
The second derivatives of the information matrix with respect to the control input $\frac{\partial^2 Q_{i,s}}{\partial [u_v]_j \partial [u_w]_k}$ is the zero matrix if $s \neq v$ or $s \neq w$, and if $s=w=v$, then
\agn*{
\frac{\partial^2 Q_{i,s}}{\partial [u_s]_j \partial [u_s]_k}   &= 
\begin{cases}
-Y_{i,s} - [r_s]_1 \frac{\partial Y_{i,s}}{\partial [u_s]_1}  &{{\rm if}}\; j= k = 1
\\
-X_{i,s} - [r_s]_2 \frac{\partial X_{i,s}}{\partial [u_s]_2}   &{{\rm if}} \begin{cases}  j= 1, k = 2 
%\\
%X_{i,s} + [r_s]_1 \frac{\partial X_{i,s}}{\partial [u_s]_1}   &{{\rm if}}\; j= 2 \and k= 1
\\
{{\rm or}}
\\
j=2, k=1
\end{cases}
\\
-Y_{i,s} - [r_s]_2 \frac{\partial Y_{i,s}}{\partial [u_s]_2}   &{{\rm if}}\;j= k = 2
\end{cases}
}
where
\agn*{
\frac{\partial Y_{i,s}}{\partial [u_s]_1} &= 
 \alpha(1-\rho) \Big( \left([\hhatx_{i,s}]_1 - [r_s]_1 - [u_s]_1 \right))
\beta_1
\Xi_1 
\\
&\hspace{2cm}+
\left([\hhatx_{i,s}]_2 - [r_s]_2 - [u_s]_2 \right)\beta_2 \Xi_2 
\Big)
\\
\frac{\partial Y_{i,s}}{\partial [u_s]_2} &= \alpha  (1-\rho)\Big(  \left([\hhatx_{i,s}]_2 - [r_s]_2 - [u_s]_2 ]\right) \beta_1
 \Xi_1 
 \\
 &\hspace{1cm}+
\left([r_s]_1 + [u_s]_1 - [\hhatx_{i,s}]_1 \right))\beta_2
\Xi_2
\Big)
}
which uses the short hand
\agn*{
\alpha &=\frac{c_0c_1 }{ \left(1 + c_1\norm{\hhatx_{i,s} - r_s - u_s}\right)^{2} \norm{\hhatx_{i,s} - r_s-u_s}}\\
\beta_1&=  \left(\frac{\alpha \left(1 + c_1\norm{\hhatx_{i,s} - r_s-u_s}\right)}
{c_0}
+
 \frac{1 }{ \norm{\hhatx_{i,s} - r_s-u_s}^2} \right)
 \\
 \Xi_1 &=  \mat{
 \cos^2 \phi_{i,s} + \rho
&
 \frac{1}{2} \sin 2\phi_{i,s}
\\
 \frac{1}{2}\sin 2\phi_{i,s}
&
  -(1+\cos^2 \phi_{i,s} )
}
\\
\beta_2&=  \frac{ 1}{\norm{\hhatx_{i,s} - r_s-u_s}^2}
 \\
 \Xi_2 &= \mat{
-\sin 2\phi_{i,s}
&
\cos 2\phi_{i,s}
\\
\cos 2\phi_{i,s}
&
\sin 2\phi_{i,s}
}
 }
 and
\agn*{
\frac{\partial X_{i,s}}{\partial [u_s]_1}
&=
([\hhatx_{i,s}]_1 - [r_s]_2 -[u_s]_2 )\Xi_3
\\
&\hspace{1cm}
-
([\hhatx_{i,s}]_2 - [r_s]_2 - [u_s]_2)\Xi_4
\\
\frac{\partial X_{i,s}}{\partial [u_s]_2} &=
([\hhatx_{i,s}]_2 - [r_s]_2 - [u_s]_2)\Xi_3
\\
&\hspace{1cm}-
([r_s]_1+[u_s]_1 - [\hhatx_{i,s}]_1)\Xi_4 .
}
where
\agn*{
\Xi_3 &= \beta_2
\left(
2 X_{i,s}
+
\alpha  \left(1 - \rho \right) \mat{
-\sin  2\phi_{i,s}
&
\cos 2\phi_{i,s}
\\
\cos 2\phi_{i,s}
&
\sin  2\phi_{i,s}
}
\right),
\\
\Xi_4 &= 2 \beta_2 X_{i,s}
\mat{0 & -1 \\ 1 & 0 }.
}
\end{prop}



==> text-16p/unused/related_work.tex <==
%Active localization using mobile sensor networks is an area of active research \cite{chung04, dames15, Gu15, esmailifar15, olfati2007distributed, vanderhook15, Adurthi13, Chung06, pereira15, 
%Distributed control of a mobile sensor network for optimal information collection can include coverage, exploration, hider-seeker games, POMDPs, active inspection, orienteering, and/or art gallery problems to spatially distributed networks of robots that rely on pairwise communication.
%In this literature review, we restrict ourselves to the subset of this literature that is directly relevant to our paper, and refer interested readers to the survey paper \cite{Skoglar07}.







There are essentially two aspects of control in this scenario -- communication and information consensus among the team \cite{kamal12,olfati2005distributed,zhou_roumeliotis11,zavlanos2008distributed} and information-theoretic motion planning \cite{olfati2007distributed,singh2007simulation,ryan2010particle,freundlich15acc,freundlich13icra,freundlich13cdc}.


Active sensing, as it applies to sensor network control, first began receiving increasing attention in 1967 under the term measurement subsystem control \cite{meier1967optimal}, where the concept of using the entires of the error covariance matrix as states in an optimal control problem was first introduced.
Active sensing and perception has been popular since the 80's \cite{bajcsy88}, but it remains an area of active research today due to its notorious difficulty.





This paper uses the distributed communication laws developed in \cite{kamal12} to inform the design of an optimal control law for the networked measurement system.
It turns out that under a linear-Gaussian dynamics assumption \cite{meier1967optimal,Hussein08,LeNy09trajectory}, the ``state'' of the system is adequately described by the pose of the sensor and the first and second order statistics of the process being estimated.
As described in \cite{freundlich15acc,Hussein08,LeNy09trajectory}, the joint space of robot poses and the statistics of the state being estimated follow a predictable trajectory governed by the joint robot motion and KF dynamical equations.
In my prior work \cite{freundlich15acc}, this predictability was exploited in order to formulate a Dynamic Program (DP) that plans measurements based on expected measurement statistics over an infinite horizon optimal control problem.

While there exists a substantial body of research on measurement control and observation planning for a single robot \cite{olfati2007distributed,singh2007simulation,ryan2010particle,freundlich15acc,freundlich13icra,freundlich13cdc,meier1967optimal,Hussein08,LeNy09trajectory,freundlich15acc}, the extension of these methods to multi robot teams has proven to be extremely difficult.
One reason for this is that planning is naturally a computationally burdensome problem, suffering from the so-called ``curse of dimensionality.''
Receding horizon control approaches, e.g., \cite{adurthi13}, can be used, however, they are limited to small action spaces and relatively short horizons compared to single robot algorithms.
%When multiple robots are involved, attempting to reason over all present and future combinations of their states in order to solve a planning instance causes an exponential increases in the number of distinct states required to represent the planning domain.
Continuous space approaches \cite{freundlich15acc,freundlich13icra,freundlich13cdc,Hussein08} are subject to local minima when searching for the optimal control input, either because they plan myopically \cite{freundlich15acc,freundlich13icra} or fall into local minima in their approach to satisfying the KF dynamics due to their non convexity \cite{Hussein08}.
The author who originally formulated the Distributed Kalman Filter (DKF) in \cite{olfati2005distributed} has extended his work to active sensing in \cite{olfati2007distributed}, but that method leads to emergent flocking behavior, which does not account with anisotropic measurement errors, a common property of real-world sensors.

